Structure effects on the giant monopole resonance and determinations of the nuclear incompressibility

Giant resonances are collective nuclear vibrations which provide a unique laboratory setting to probe the bulk properties of the nuclear force. One of the isoscalar compressional modes -- the isoscalar giant monopole resonance (ISGMR) -- is useful in constraining the equation of state (EoS) of nuclear matter. For example, the nuclear incompressibility, $K_\infty$, is a fundamental quantity in the EoS and is directly correlated with the energies of the ISGMR in finite nuclei. Previous work has shown that interactions with $K_\infty$ which reproduce the energies of the ISGMR in $^{208}$Pb and $^{90}$Zr well, overestimate those of the tin and cadmium nuclei. To further investigate where this "softness" appears in moving away from the doubly-closed nucleus $^{90}$Zr, and how this effect develops, the first portion of this thesis consists of measurements of the ISGMR in the molybdenum isotopes. Comparison of the ISGMR strengths with Random Phase Approximation calculations shows that these nuclei have ISGMR energies which are overestimated to a similar degree as seen in the tin and cadmium nuclei, while the strength of $^{208}$Pb is precisely reproduced. This suggests clearly that the molybdenum nuclei exhibit the same open-shell softness which has been documented previously. The ISGMR in isotopes encompassing a broad range of proton-neutron asymmetries constrains the dependence of the nuclear incompressibility on the isospin asymmetry, as quantified by the asymmetry term, $K_\tau$. To reconcile previously-published and highly concerning conclusions that $K_\tau = + 582$ MeV, the second portion of this thesis is focused upon independently studying this claim. A simultaneous measurement of the ISGMR in $^{40,42,44,48}$Ca has excluded the possibility of a positive value for $K_\tau$, and found consistency with previous data, placing $K_\tau$ at $-510 \pm 115$ MeV.

==> calibration.tex <==
%
% Modified by Megan Patnott
% Last Change: Jan 18, 2013
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Modified by Sameer Vijay
% Last Change: Tue Jul 26 2005 13:00 CEST
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Sample Notre Dame Thesis/Dissertation
% Using Donald Peterson's ndthesis classfile
%
% Written by Jeff Squyres and Don Peterson
%
% Provided by the Information Technology Committee of
%   the Graduate Student Union
%   http://www.gsu.nd.edu/
%
% Nothing in this document is serious except the format.  :-)
%
% If you have any suggestions, comments, questions, please send e-mail
% to: ndthesis@gsu.nd.edu
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% Appendix 1
%

\chapter{Energy calibration of the focal plane}  \label{experimental:energy_calibration}

The scattered particles were accepted into Grand Raiden and subsequently dispersed laterally according to their magnetic rigidity due to the presence of the dipole fields of the D1 and D2 elements of the spectrometer. The charged particle with mass $m$ and charge $q$ moving  relativistically ($\gamma = 1/\sqrt{1-v^2}$) through and perpendicular to a magnetic field $B$ will be bent through a circular arc of radius $\rho$. As such, with the magnetic fields and velocity being perpendicular to one another, the Lorentz force results in uniform circular motion for a magnetic rigidity $[B \rho]$:
\begin{align}
  \frac{\gamma m v^2}{\rho} &= q v B \notag \\
  [B \rho] &= \frac{\gamma m v}{q} \notag \\
  &= \frac{p}{q}.
  \label{mag_rigidity}
\end{align}
Bearing this in mind as well as the geometry of Grand Raiden (cf. Fig. \ref{GR}) suggests that $\alpha$-particles which have higher momenta -- thereby having transferred less momentum to the recoiling target nucleus -- will have greater radii of curvature in their trajectories through the spectrometer. Inversely, $\alpha$-particles which have lower momenta will have smaller radii of curvature in their trajectory. The observable implication of this is that higher-momentum $\alpha$-particles, which have left the recoiling nucleus with a smaller excitation energy, will be detected further to the outside of the focal plane, whereas lower-momentum $\alpha$-particles will be detected closer to the interior edge of the focal plane. In this way, the position at which the incident $\alpha$-particles were detected at the focal plane is directly related to the particle momentum, and extensibly, the excitation energy of the recoiling target nucleus.

%As such, the utility of the position dependence of the focal plane detection system is made clear.

The general procedure for the momentum calibration of the focal plane is to take a species with known excitations, and to calculate the corresponding $\alpha$-momenta which would leave the recoiling calibrant nucleus in its excited states. Upon doing so, one can then precisely empirically determine the functional dependence $p(X_\text{fp})$ which describes the dispersion of the focal plane momentum across the lateral dispersion plane. This is a property \emph{only} of the magnetic field settings of the spectrograph, and indeed scales directly with the field strength as seen in Eq. \eqref{mag_rigidity}.

For each experiment, \nuc{24}{Mg} was used as the calibration nucleus owing to high-quality reference spectra obtained from Ref. \cite{Kawabata_private}. Figure \ref{24Mg_calibration} shows a sample post-calibration spectrum of \nuc{24}{Mg} at the zero-degree setting of Grand Raiden.

\begin{figure*}[t!]
\includegraphics[width=\linewidth]{./figures/experimental_figures/24Mg_0deg_withMomentum.pdf}
\caption[Sample $0^\circ$ calibration spectra for \nuc{24}{Mg}($\alpha,\alpha^\prime$).]{Sample $0^\circ$ calibration spectra for \nuc{24}{Mg}($\alpha,\alpha^\prime$), showing both the calibrated excitation energy as well as the detected $\alpha$-particle momentum after calibration. }
\label{24Mg_calibration}
\end{figure*}





\begin{figure*}[t!]
\includegraphics[width=\linewidth]{./figures/experimental_figures/kinematics_figure.pdf}
\caption[Sketch of the forward-kinematics scattering process.]{Sketch of the forward-kinematics scattering process in the laboratory frame, with the scattering angle $\theta$ shown.}
\label{kinematics_figure}
\end{figure*}

For a two-body reaction $A_1 + A_2 \rightarrow A_3 + A_4$ with the target nucleus $A_1$ starting from rest, the kinematics are sketched in Fig. \ref{kinematics_figure}.  With the incident projectile leaving the target nucleus with a recoil 4-momentum $p_4$ and leaving with itself a 4-momentum of $p_3$, the relativistic conservation of 4-momentum holds. The initial momentum of the system is:
\begin{align}
  p_i &= p_1 + p_2 \notag \\
  &= (m_1,\vec{0}) + (E_2,\vec{p}_2).
\end{align}
Similarly, the final momentum of the system is:
\begin{align}
  p_f & = p_3 + p_4 \notag \\
  &= (E_3,\vec{p}_3) + (E_4,\vec{p}_4).
\end{align}

The initial momentum of the incident $\alpha$ beam is known from the beam energy at the scattering site:
\begin{align}
  E_1^2 &= \vec{p}_1^2 + m_1^2 \notag \\
  (E_\text{beam}+m_1)^2 &= \vec{p}_1^2 + m_1^2 \notag \\
  p_1 & = \sqrt{E_\text{beam}^2 + 2 m_1 E_\text{beam}}
\end{align}

With the aforementioned calibration reference spectra of \nuc{24}{Mg}, the momentum $\vec{p}_3$ is directly measured and in so doing, the total energy $E_3$ of the ejectile is also measured:
\begin{align}
  E_3 = \sqrt{\vec{p}_3^2 + m_3^2}.
\end{align}

Furthermore, the total 3-momentum of the ejectile and recoiling target is conserved relative to that of the incident projectile and stationary target. As such, inspection of Fig. \ref{kinematics_figure} shows that the 3-momenta $\vec{p}_3$, $\vec{p}_4$, and $\vec{p}_2 = \vec{p}_3+\vec{p}_4$ constitute a triangle for which the law of cosines defines the recoil momentum in terms of the laboratory-frame scattering angle of $\vec{p}_3$ relative to the beam axis:
\begin{align}
  \vec{p}_4^2 &= \left(\vec{p}_3 + \vec{p}_4 \right)^2 + \vec{p}_3^2 - 2 \left(\vec{p}_3 + \vec{p}_4 \right) \cdot \vec{p}_3 \notag \\
  &= \vec{p}_2^2 + \vec{p}_3^2 - 2 | \vec{p}_2 | | \vec{p}_3| \cos \theta. \label{recoil_momentum}
\end{align}

Inspection of the energy component of the 4-momentum conservation equations yields:
\begin{align}
  m_1 + (m_2 + E_\text{beam}) &= E_3 + E_4, \label{recoil_mass}
\end{align}
and the corresponding invariant interval for $p_4$ yields
\begin{align}
  E_4^2 & = \vec{p}_4^2 + m_4^2. \label{recoil_interval}
\end{align}

In terms of the excitation energy $E_x$, $m_4 = m_1+E_x$, and thus the latter equation yields the excitation in terms of the previously derived quantities in Eqs. \eqref{recoil_momentum} and \eqref{recoil_mass}:
\begin{align}
  E_x = \sqrt{E_4^2 - \vec{p}_4^2} - m_2.
  \label{excitation_energy_formula}
\end{align}

Equations \eqref{recoil_momentum}-\eqref{excitation_energy_formula} were applied event-wise to each data set using the $p_3(X_\text{fp})$ function constrained by the reference \nuc{24}{Mg} spectra taken at the same magnetic field and angular settings of the spectrograph. Using Eq. \eqref{mag_rigidity}, any fluctuation in the dipole field strengths between runs were accounted for in the extracted $p_3(X_\text{fp})$ function via proportional scaling of the fit functions by the dipole strengths. Finally, despite the energy losses through the target foil being small ($\sim 1$ keV), they were nonetheless accounted for using the statistical SRIM framework \cite{SRIM}.



% \bibliographystyle{ndnatbib}
% \bibliography{example}

